Hierarchical Weight Averaging for Deep Neural Networks

Despite the simplicity, stochastic gradient descent (SGD)-like algorithms are successful in training deep neural networks (DNNs). Among various attempts to improve SGD, weight averaging (WA), which averages the weights of multiple models, has recently received much attention in the literature. Broadly, WA falls into two categories: 1) online WA, which averages the weights of multiple models trained in parallel, is designed for reducing the gradient communication overhead of parallel mini-batch SGD, and 2) offline WA, which averages the weights of one model at different checkpoints, is typically used to improve the generalization ability of DNNs. Though online and offline WA are similar in form, they are seldom associated with each other. Besides, these methods typically perform either offline parameter averaging or online parameter averaging, but not both. In this work, we firstly attempt to incorporate online and offline WA into a general training framework termed Hierarchical Weight Averaging (HWA). By leveraging both the online and offline averaging manners, HWA is able to achieve both faster convergence speed and superior generalization performance without any fancy learning rate adjustment. Besides, we also analyze the issues faced by existing WA methods, and how our HWA address them, empirically. Finally, extensive experiments verify that HWA outperforms the state-of-the-art methods significantly.

==> HWA (2)/HWA.tex <==

\section{Detailed Procedure of HWA}
\label{sec:hwa}
In this section, we  introduce the detailed procedure of HWA and  leave the analysis of how HWA works in Section~\ref{sec:discuss}.  The general idea of HWA is given in Figure~\ref{fig:L123}(c).  In Algorithm~\ref{alg:hwa1} and \ref{alg:hwa2}, we also provide the  pseudo-code  of the  online   and  offline  modules of HWA, respectively.   










\subsection{Online Module of HWA} At the online stage,  HWA trains $K$ models in parallel  with different  sampling orders. A standard SGD optimizer $\mathcal A$ with a regular decaying learning rate scheduler  is used to evolve each model by performing $H$ sequential SGD updates to batches of  training examples $\psi$ sampled from the dataset $\mathcal D$:
\begin{align*}
\overbrace{\mathbf W^k_{e,t}}^{{\emph{Inner  Weights}}}&\leftarrow \mathbf W^k_{e,t-1}+\mathcal A\left(\mathcal L, \mathbf W^k_{e,t-1},\psi_{e,t}^k\right)\\
\mbox{where~}&k\in\{1,2,\ldots, K\}~,t\in \{1,2,\ldots, H\}
\end{align*}
Here $\mathcal L$ is the loss function, and $e$ denotes $e_{th}$  averaging or synchronization cycle.   After   each model is updated for $H$ iterations ($\mathbf W^k_{e,0}\rightarrow \mathbf W^k_{e,H}$), HWA takes the average of the weights of the $K$ models in parallel  to obtain the averaged weights for the $e_{th}$ synchronization cycle
$$
\overbrace{\overline{\mathbf W}_{e}}^{\emph{Outer  Weights}}=\frac{\sum_{k=1}^K\mathbf W_{e,H}^k }{K}
$$
Once completed, it  synchronizes  the weights of each model at the start of the next synchronization cycle $\mathbf W_{e+1,0}^k$ to the averaged weights
$$
\mathbf W_{e+1,0}^k\leftarrow \overline{\mathbf W}_{e}~\mbox{~where~}k\in\{1,2,\ldots, K\}
$$
Since   $\mathbf W_{e+1,t}^k$ is updated within a synchronization cycle and $\overline{\mathbf W}_{e}$ is calculated outside of a synchronization cycle, we name them \emph{Inner Weights} and \emph{Outer Weights}, respectively.   

\begin{algorithm}[h!]
    \caption{Online Module of HWA}
    \label{alg:hwa1}
    \KwIn{Synchronization Period $H$, Optimizer $\mathcal A$, Loss Function $\mathcal L$, Number of Models $K$,  Maximum Iterations  $T$}
    % \KwOut{Online averaged weight $\mathbf W^O$}
    Initialize Inner Weight $\mathbf W_{0,0}^k$ for $k\in\{1,2,\ldots, K\}$\\
    \For{$i = 1$ to $T$}{
        $e\leftarrow \lfloor (i-1)/H\rfloor$  ($e_{th}$ synchronization cycle)\\
        $t\leftarrow  i-e\times H$ ($t_{th}$ step in the $e_{th}$ synchronization cycle)\\
     
        \For{k = 1 to $K$}{
            Sample a batch of data $\psi_{e,t}^{k}$ for model $k$ \\
            $\mathbf W_{e,t}^k\leftarrow \mathbf W_{e,t-1}^k+\mathcal A\left(\mathcal L, \mathbf W_{e,t-1}^k,\psi_{e,t}^k\right)$\\
        }
        \If{$t=H$}{
            $\overline{\mathbf W}_{e}=\frac{\sum_{k=1}^K\mathbf W_{e,t}^k }{K}$\\
            Save checkpoint $\overline{\mathbf W}_{e}$\\
          \For{k = 1 to $K$}{
               $\mathbf W_{e+1,0}^k\leftarrow \overline{\mathbf W}_{e}$\\
            }
          }
    }
\end{algorithm}



% The inner weights $\mathbf W^{I}$ are updated through applying   to batches of  training examples $\psi$ sampled from the dataset $\mathcal D$. The  optimizer $\mathcal A$ evolves network $\mathbb N_i$ by taking $H$ sequential  updates  with mini-batch size $B$ in \emph{the inner loop}:




% Once the inner weights is updated for each network,  the outer weights of each network $\mathbf W_e^O$ is updated to the average of  multiple inner weights $\{\mathbf W_e^I(i)\}_{i=1}^m$.







% The convergence guarantees of on-line trajectory averaging was analyzed in ~\cite{zhang2019lookahead}.




%  \begin{figure}[h!]
% \centering
% \includegraphics[width=0.5\textwidth]{draw/3.png}
      
% \caption{The training accuracy  of MobileNetV2 on Cifar 100 for two successive averaging rounds. }
% \label{fig:exp1}
% \end{figure}
% Figure~\ref{fig:exp1} shows training accuracy  of MobileNetV2 on CIFAR-100 for two successive epochs.


% While the inner weights are exploring around the minima,  online averaging enables  the network to quickly progress to a deeper position on the loss landscape.



 




% The SWA algorithm is able to find a point centered in the region of optimal points on the loss surface by averaging the solutions of SGD with a constant or cyclical learning rates at the end of training course.   Inspired by SWA,

\subsection{Offline  Module of HWA}  At the offline stage,  HWA also further averages the outer weights $\overline{\mathbf W}_e$  saved at different synchronization  cycles during the online stage.  Unlike offline WA,  HWA does not require  a large  constant or cyclical learning rate at the end of the training process.   From our experiments,  we find it works well with a regular decaying learning rate scheduler over the entire budget, \eg, a cosine decay or linear decay. 

While offline WA averages all the model checkpoints sampled from the time it starts averaging, HWA uses a slide window with a length of $I$ and  takes the average of outer weights  at  different synchronization cycles within the window. 
\begin{align*}
\overbrace{\overline{\overline{\mathbf W}}_{e}}^{\emph{HWA Weights}}=\frac{\sum_{t=e-I+1}^{e}}{I} \overline{\mathbf W}_{t}
\end{align*}
In practice,   the offline WA module does not necessarily average all the outer weights $\overline{\mathbf W}_{e}$ within the slide window. For example, it can take the average of  outer weights $\overline{\mathbf W}_{e}$ with index in multiples of a particular integer, \eg, $\{\overline{\mathbf W}_{3},\overline{\mathbf W}_{6},\overline{\mathbf W}_{9},\ldots\}$.  Besides, when we have sufficient training budget,   we can try multiple  possible $I\in \mathbb I=\{I_1,I_2,\ldots\}$  as the length of slide window also has a significant impact on the performance of the final averaged model $\overline{\overline{\mathbf W}}_{e}$.
\begin{algorithm}[h!]
    \caption{Offline  Module of HWA}
    \label{alg:hwa2}
    \KwIn{ Checkpoints of Outer Weights $\overline{\mathbf W}_e$ for $e\in \{1,2,3...\}$, Slide Window Length $I$.}
    
    \For{$e = 1,2,\ldots$}{
   $\overline{\overline{\mathbf W}}_{e}=\frac{\sum_{t=e-I+1}^{e}}{I} \overline{\mathbf W}_{t}$\\
    Update batch normalization statistics if the DNN uses batch normalization
    }
\end{algorithm}

 
\section{How HWA Works?}
\label{sec:discuss}

In this section, we   discuss how  HWA  improves the training efficiency and  generalization ability of DNNs. 
\subsection{Convergence Condition of SGD} 
\label{sec:convsgd}

In order to study how HWA improves SGD, here  we first derive the convergence condition of SGD.  Let $R_N(\mathbf W_{e,t})=\frac{1}{N}\sum_{i=1}^N \mathcal L(\mathbf W_{e,t},\psi_i)$ denote the empirical risk of model  $\mathbf W_{e,t}$ and $\psi_i=(x_i,y_i)$ denote a single training sample.  Suppose the batch size is $B$, then the gradient of a batch of samples is  $$
g(\mathbf W_{e,t},{\psi}_{e,t})=\frac{1}{B}\sum_{i=1}^B \nabla_{W} \mathcal L(\mathbf W_{e,t},{\psi}_{i})\approx \nabla_W R_N(\mathbf W_{e,t})$$
On the assumption of Lipschitz-continuous gradient with Lipschitz constant $L$ and the update  at each iteration is $\Delta W=-\eta g(\mathbf W_{e,t},{\psi}_{e,t})$, we have 

\begin{align*}
&||\nabla_W R_N(\mathbf W_{e,t}+\Delta W)-\nabla_W R_N(\mathbf W_{e,t})||\leq L ||\Delta W||_2\\
 %&\mbox{where L is lipschitz constant}.\\
\Rightarrow  &  R_N(\mathbf W_{e,t}+\Delta W)- R_N(\mathbf W_{e,t}) \\ & \leq  \frac{1}{2}L ||\Delta W||_2^2+\nabla_W R_N(\mathbf W_{e,t})^T \Delta W\\
%& \mbox{At iteration t, the update is }\Delta W=-\eta g(\mathbf W^I_{e,t},{\psi}_{e,t})\\
\Rightarrow  &  R_N(\mathbf W_{e,t+1})- R_N(\mathbf W_{e,t})\\ &\leq \frac{1}{2}L \eta^2 || g(\mathbf W_{e,t},{\psi}_{e,t})||_2^2-\eta \nabla_W R_N(\mathbf W_{e,t})^T g(\mathbf W_{e,t},{\psi}_{e,t}),\\
% \Rightarrow &  \mathbb E_{\Psi_{e,t}}\left[ R_N(\mathbf W^I_{e,t+1}) \right]-R_N(\mathbf W^I_{e,t})\\
% &\leq \frac{1}{2}L \eta^2\mathbb E_{\Psi_{e,t}}\left[||g(\mathbf W^I_{e,t},\Psi_{e,t}))||_2^2\right] \\
% &  -\eta \nabla_W R_N(\mathbf W^I_{e,t})^T  E_{\Psi_{e,t}}\left[g(\mathbf W^I_{e,t},\Psi_{e,t}))\right]
\end{align*}

Suppose $\Psi_{e,t}$ denotes the variable of  mini-batch samples,  the empirical risk is expected to decrease  if 
\begin{align*}
 & \mathbb E_{\Psi_{e,t}}\left[ R_N(\mathbf W_{e,t+1})\right]-R_N(\mathbf W_{e,t}) \leq 0\\
 \Rightarrow & \frac{1}{2}\eta L \mathbb E_{\Psi_{e,t}}\left[||g(\mathbf W_{e,t},\Psi_{e,t})||_2^2\right] \\
 & - \nabla_W R_N(\mathbf W_{e,t})^T \mathbb E_{\Psi_{e,t}}\left[g(\mathbf W_{e,t},\Psi_{e,t})\right]\leq 0\\
  \Rightarrow &\frac{1}{2}\eta L ||\mathbb E_{\Psi_{e,t}} \left[g(\mathbf W_{e,t},\Psi_{e,t})\right]||^2_2 \\&+\frac{1}{2}\eta L \mathbb E_{\Psi_{e,t}}[||g(\mathbf W_{e,t},\Psi_{e,t})-\nabla_W R_N(\mathbf W_{e,t})||_2^2]&\\& \leq  \nabla_W R_N(\mathbf W_{e,t})^T \mathbb E_{\Psi_{e,t}}\left[g(\mathbf W_{e,t},\Psi_{e,t})\right]\\
  \Rightarrow & \frac{1}{2} L \mathbb E_{\Psi_{e,t}}[||g(\mathbf W_{e,t},\Psi_{e,t})-\nabla_W R_N(\mathbf W_{e,t})||_2^2]\\& \leq 
  (\frac{1}{\eta}-\frac{1}{2} L)||\nabla_W R_N(\mathbf W_{e,t})||^2_2
\end{align*}
For a fixed dataset $\mathcal D$ and model $\mathbf W_{e,t}$,  the right hand side  $(\frac{1}{\eta}-\frac{1}{2} L)||\nabla_W R_N(\mathbf W_{e,t})||^2$ is determined by the learning rate $\eta$,  and left hand side $ \frac{1}{2} L \mathbb E_{\Psi_{e,t}}[||g(\mathbf W_{e,t},\Psi_{e,t})-\nabla_W R_N(\mathbf W_{e,t})||_2^2]$ is controlled by the batch size.  As long as the learning rate $\eta$ stays constant,  model $\mathbf W_{e,t}$ would converge only if the mini-batch gradient $g(\mathbf W_{e,t},\Psi_{e,t})$ estimates $\nabla_W R_N(\mathbf W_{e,t})$ accurately enough. 
\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{newplot/constlr.png}
\caption{The top-1 accuracy of ResNet20 on CIFAR100 with different constant learning rates.
}
\label{fig:constlr}
\end{figure}


Therefore, with a constant learning rate $\eta$, the optimizer would converge to a certain point and then start to oscillate and  explore around the minima.  This phenomenon is clearly shown in Figure~\ref{fig:constlr}, where we plot the training and test accuracy of ResNet20 on CIFAR100 when it is trained by SGD with a constant learning rate $\eta\in \{0.1,0.25\}$. As we can see, the training and test accuracy start to oscillate  after dozens of epochs, which indicates that the optimizer is exploring around the local minima instead of progressing  to the local minima.


\subsection{How HWA Improves Training Efficiency} 
\label{sec:discussefficiency}
Though  the loss functions of DNNs are known to be nonconvex~\cite{choromanska2015loss}, the loss surfaces  over the trajectory of SGD are approximately convex~\cite{goodfellow2014qualitatively}. According to the convergence condition,  SGD would oscillate and explore around the local minima after it converges to a certain point unless the learning rate $\eta$ further decays.  Therefore,  by taking the average of the weights of multiple model checkpoints, the averaged solution would  quickly progress to a point  closer to the minima with training lower loss.


This scenario is shown in  Figure~\ref{fig:onlinewavis}, where we use the visualization tool~\cite{li2018visualizing}  to project  model checkpoint  $\mathbf W^1_{101,H}$ and $\mathbf W^2_{101,H}$ (two models in parallel)  and their corresponding averaged weights $\overline{\mathbf W}_{101}$ on the training loss surface of ResNet32 on CIFAR100. Note that,  $\mathbf W^1_{101,H}$ and  $\mathbf W^2_{101,H}$ are evolved by SGD for $H=391$ steps (one epoch) from the same starting point  $\overline{\mathbf W}_{100}$, and hence they are within the same local minima. Through the online averaging operation, the averaged solution $\overline{\mathbf W}_e$ immediately reaches  a location closer to the minima on the training loss surface.
\begin{figure}[t!]
        \centering
        \includegraphics[width=0.35\textwidth]{newplot/onlinewavis.pdf}
        \caption{The projection of  the online averaging operation of HWA on the training loss surface of ResNet32 on CIFAR100.}
        \label{fig:onlinewavis}
\end{figure}

Similar to the online averaging operation of HWA,  the offline averaging operation of HWA also speeds up convergence in a similar way.  However as the offline averaging operation of HWA  is performed vertically at different synchronization cycles on top of  the outer weights $\overline{\mathbf W}_e$ obtained during the online stage,  the  HWA weights  $\overline{\overline{\mathbf W}}_e$  progresses to a point  closer to the minima than  $\overline{\mathbf W}_e$.  To  show  this scenario, we also use the visualization tool~\cite{li2018visualizing} to project the offline averaging operation of HWA in Figure~\ref{fig:offlinewavis}. 

\begin{figure}[t!]
        \centering
        \includegraphics[width=0.35\textwidth]{newplot/offlinewavis.pdf}
        \caption{The projection of the offline averaging operation of HWA on the training loss surface of ResNet32 on CIFAR100.}
        \label{fig:offlinewavis}
\end{figure}

Therefore,  by performing the weight  averaging operations  in both  horizontal and vertical directions  hierarchically, HWA can progress to the local minima more quickly than online WA alone, which only performs the averaging operation horizontally. In Figure~\ref{fig:mobv2}, we plot the top-1 test accuracy and test loss of \emph{Inner Weights} $\mathbf W_{e,H}^k$, \emph{Outer Weights} $\overline{\mathbf W}_e$, and  \emph{HWA Weights} $\overline{\overline{\mathbf W}}_e$ for ResNet32 on CIFAR10 and CIFAR100, where the synchronization period is $H=391$ (\ie, one epoch) and  the length of slide window is $I=20$. As we can observe,  the \emph{HWA Weights}  $\overline{\overline{\mathbf W}}_e$  achieves faster convergence than \emph{Outer Weights} $\overline{\mathbf W}_e$ and inner weights  $\mathbf W_{e,H}^k$.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{newplot/r32converge.png}
\caption{Top-1 test accuracy and test loss of  \emph{Inner Weights} $\mathbf W_{e,H}^k$, \emph{Outer Weights} $\overline{\mathbf W}_e$, and  \emph{HWA Weights} $\overline{\overline{\mathbf W}}_e$ for ResNet32 on CIFAR10 and CIFAR100. The learning rate decays along a cosine curve.
% A silde window with a length of 20 epochs is used in the offline averaging stage. 
}
\label{fig:mobv2}
\end{figure}





%  ~\begin{table}[h!]
% \tiny
%   \centering
%   \setlength{\tabcolsep}{1.1mm}{
%   \begin{tabular}{cccccc}
%      \toprule[1pt]
%  ResNet20        &  ResNet32  &  ResNet56&  ResNet110 &  VGG16 & MobileNetV2\\

%   $93.36\pm 0.18$ &$94.39\pm 0.05$  & $94.74\pm 0.19$&  $94.89\pm 0.29$  & $94.83\pm 0.05$  & $95.03\pm 0.16$\\
% $70.62\pm 0.11$  & $73.11\pm 0.05$ & $75.25\pm 0.31$ &$76.62\pm 0.25$  &$76.92\pm 0.27$  & $76.79\pm 0.39$ \\
%      \toprule[1pt]
%   \end{tabular}
%  }
% %   \caption{Statistic Result }
%   \label{tab:stat}
% \end{table}



 
\subsection{How HWA Improves Generalization Ability}
\label{sec:discussgeneralization}
One popular hypothesis about  the \emph{\textbf{generalization ability}}\footnote{In this paper, we refer to  generalization ability as the ability  in predicting unseen, \emph{in-distribution} data (\eg, test data).}  of DNNs~\cite{cooper2018loss,draxler2018essentially,izmailov2018averaging} is that  the generalization performance of DNNs is correlated with the flatness of its local minima, and a sharp local minimum typically tends to generalize worse than the flat ones~\cite{keskar2016large}.  While most existing works (\eg,~\cite{izmailov2018averaging,zhang2019your}) attribute the better generalization ability of neural networks to a wider local minimum,  the location to which a network converges within  a local minimum also  greatly affects  the generalization performance.   As observed in~\cite{he2019asymmetric},  the loss landscape of  local minima is asymmetric and exists both sharp and flat directions, and the solution locates at the flat side has better generalization performance due to  the  random shift between the  training loss and test loss.



\begin{figure}[t!]
\centering
\includegraphics[width=0.4\textwidth]{newplot/biasflat.pdf}
\caption{A simple illustration of  why averaged model tends to be biased to the flat side of the local minima.
}
\label{fig:biasflat}
\end{figure}

According to the convergence condition of SGD, when the model checkpoints are sampled with the same learning rate, they would be  distributed around  the local minima with similar empirical risks  (refer to Figure~\ref{fig:constlr}).  As a result, as illustrated in Figure~\ref{fig:biasflat},  the averaged model  tends to be  biased to the flat side of the local minima.  Due to the  shift between the training and test loss, the averaged model has better generalization ability than the model with the minimal training loss.  Such an example is shown in  Figure~\ref{fig:asymmetric}, which   plots  the accuracy and loss of ResNet20 on CIFAR100 along the direction between an averaged model   (location $x=0$) and an individual model   (location $x=1$).  Apparently,  all the models  between  $x=0$ and  $x=1$ are in the same local minima because there is no sharp drop in  training and test accuracy.  Despite the lower training accuracy,   the  averaged model  achieves higher test accuracy than the individual model, because it is biased to the  flat side of the loss landscape. This also implies that the training accuracy  is a poor indicator of the generalization ability.

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{newplot/asymmetric.pdf}
\caption{The accuracy and loss   on CIFAR100 along the direction between an averaged model (location $x=0$) and an individual model (location $x=1$).
}
\label{fig:asymmetric}
\end{figure}





Figure~\ref{fig:biasflat} also explains why offline WA is sensitive to the choice of learning rate used to sample model checkpoints. According to the convergence condition of SGD, the learning rate determines the empirical risk or loss of the sampled  model checkpoints (refer to Figure~\ref{fig:constlr}) and hence their locations on the loss landscape. Since the averaged model is obtained by taking the average of these model checkpoints, its  location within the local minima is also determined by the learning rate with which these model checkpoints are sampled.   As a result, a choice of learning rate that is either too small or too large  can be detrimental to  the  performance of offline WA, which leverages  a large constant or cyclical learning rate to sample model checkpoints. For example  in   Figure~\ref{fig:biasflat}, the averaged model obtained with an intermediate learning rate achieves the best test performance.

\begin{figure}[t!]
\centering
\includegraphics[width=0.35\textwidth]{newplot/biasflat2.pdf}
\caption{The averaged model $\overline{\overline{\mathbf W}}_e$ at different  synchronization cycles is located at different positions on the loss landscape  
}
\label{fig:biasflat2}
\end{figure}

Unlike offline WA, as illustrated in Figure~\ref{fig:biasflat2}, HWA  takes the average of  model checkpoints  sampled with different learning rates  with a slide window of length $I$.  As a result, the averaged model $\overline{\overline{\mathbf W}}_e$ at different synchronization cycles is located at different positions  with different distances to the minima of the training loss surface.  Compared to offline WA,  HWA is able to explore more locations on the flat side of the local minima and hence is more likely  to find a better averaged model.  

Note that, the averaged model at the last synchronization cycle does not necessarily be the best averaged model. For example, as illustrated in Figure~\ref{fig:biasflat2}, the best averaged model  $\overline{\overline{\mathbf W}}_7$ is obtained at the $7_{th}$ synchronization cycle.  We also plot the training and test  accuracy of $\overline{\overline{\mathbf W}}_e$ as a function of epochs  for ResNet110 on CIFAR100 in Figure~\ref{fig:biasflat3}, where the synchronization period is one epoch and the length of slide window $I=20$. As we can observe, the  averaged model   $\overline{\overline{\mathbf W}}_e$  around the $150_{th}$ synchronization cycle achieves the best test accuracy.  Therefore, in practice, we  use techniques such as early stopping  to obtain the best averaged model.

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{newplot/biasflat3.pdf}
\caption{The training and test accuracy of $\overline{\overline{\mathbf W}}_e$ as a function of epoch (the synchronization period is one epoch) for ResNet110 on CIFAR100.
}
\label{fig:biasflat3}
\end{figure}

Though the averaged model with the minimal training loss   does   not necessarily be  the averaged model with the best validation performance, in most cases,  the best averaged model is  located close to the minima of the training loss.  Therefore, it is important for the optimizer to explore more locations close to the  minima of the training loss.  With the help of the online WA module,  HWA progresses to  the regions
close to the minima of training loss more quickly than naive offline WA, which as a result,  helps it to find  a better averaged model.


\noindent \textbf{Discussion:}  The   ‘restart’ mechanism~\cite{loshchilov2016sgdr,smith2017cyclical},  which switches the status of a  model to a lower fitting level to the training data (\ie, higher training loss),  is claimed to achieve a longer-term beneficial effect on generalization performance at the cost of short term benefit. While existing techniques~\cite{loshchilov2016sgdr,smith2017cyclical} restart the training by increasing the learning rate, we observe that the online averaging module of HWA  also achieves a similar  `restart' effect. We observe  that, in general, the loss of the averaged model $\overline{\overline{\mathbf W}}_e$ decreases over training time.  However,   within a synchronization cycle,  the loss of  inner weights $\mathbf W_{e,t}^k$ would surprisingly increase with iteration times $t$.  For example, as shown in Figure~\ref{fig:restart}, after  each model is updated by the optimizer for $H$ steps ($\mathbf W_{100,0}^k\rightarrow \mathbf W_{100,H}^k $), the training loss increases instead of decreasing.
\begin{figure}[h!]
\centering
\includegraphics[width=0.35\textwidth]{newplot/restart.pdf}
\caption{The projection  of the  `restart' effect of HWA  on the training loss surface of ResNet32 on CIFAR100
}
\label{fig:restart}
\end{figure}

Note that  the online averaging operation of HWA would result in a significant decrease in the empirical risk, \ie, 
\begin{align*}
R_N(\overline{\mathbf W}_e)&\ll R_N(\mathbf W_{e,H}^k),~
 \mathbf W_{e+1,0}^k \leftarrow \overline{\mathbf W}_e\\
 \Rightarrow &R_N(\mathbf W_{e+1,0}^k)\ll R_N(\mathbf W_{e,H}^k)
\end{align*}
As a result, the convergence condition  at the start of  the $e+1_{th}$ synchronization cycle does not hold any more for $\mathbf W_{e+1,0}^k$, and the optimizer $\mathcal A$ would receive more noise information than gradient information within the synchronization cycle. That's why the empirical risk $R_N(\mathbf W_{e+1,t}^k)$ increases in general with the iteration  times $t$ within a synchronization cycle. 

While there  is no consensus on  how the `restart' mechanism improves the training of DNNs,   we provide a possible explanation to the success of the  `restart' mechanism:  A neural network tends to generalize  easy training samples  and   memorizes the  ``hard'' samples through the massive parameters.   Once the  hard samples are memorized, their losses would  decrease to zero quickly, and hence the network  overfits the hard samples.  On the other hand, restart techniques switch the network status back  to a lower fitting level,  and hence the hard samples memorized by the network  are more likely  to be forgotten.  












